Hydra Attention: Efficient Attention with Many Heads

While transformers have begun to dominate many tasks in vision, applying them to large images is still computationally difficult. A large reason for this is that self-attention scales quadratically with the number of tokens, which in turn, scales quadratically with the image size. On larger images (e.g., 1080p), over 60% of the total computation in the network is spent solely on creating and applying attention matrices. We take a step toward solving this issue by introducing Hydra Attention, an extremely efficient attention operation for Vision Transformers (ViTs). Paradoxically, this efficiency comes from taking multi-head attention to its extreme: by using as many attention heads as there are features, Hydra Attention is computationally linear in both tokens and features with no hidden constants, making it significantly faster than standard self-attention in an off-the-shelf ViT-B/16 by a factor of the token count. Moreover, Hydra Attention retains high accuracy on ImageNet and, in some cases, actually improves it.

==> figures/6_interleave.tex <==
% \begin{figure}[t]
% \begin{center}
% 	\includegraphics[width=0.6\linewidth]{figures/images/interleave.png}
%     \caption{\textbf{Interleaving Hydra Attention.} Interleaving Hydra attention layers compared to simply replacing them starting with the last layer as in Fig.~\ref{subfig:backward_scan}. When interleaving, we always replace the last layer, and don't replace the first layer. Then we evenly intersperse the rest of the layers. Thus, 6 layers would replace every other layer.}
% 	\label{fig:interleave}
% \end{center}

% \end{figure}
